Linear functional classes over cellular automata

Cellular automata are a discrete dynamical system which models massively parallel computation. Much attention is devoted to computations with small time complexity for which the parallelism may provide further possibilities. In this paper, we investigate the ability of cellular automata related to functional computation. We introduce several functional classes of low time complexity which contain "natural" problems. We examine their inclusion relationships and emphasize that several questions arising from this functional framework are related to current ones coming from the recognition context. We also provide a negative result which explicits limits on the information transmission whose consequences go beyond the functional point of view.

==> eptcsdata.tex <==
\providecommand{\firstpage}{177}
\providecommand{\publicationstatus}{E. Formenti (Ed.): AUTOMATA and JAC 2012 conferences\\
EPTCS 90, 2012, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.90.15}{10.4204/EPTCS.90.15}}
\pdfoutput=1

